DexGraspNet 2.0: Learning Generative Dexterous Grasping in Large-scale Synthetic Cluttered Scenes

Grasping in cluttered scenes remains highly challenging for dexterous hands due to the scarcity of data. To address this problem, we present a large-scale synthetic benchmark, encompassing 1319 objects, 8270 scenes, and 427 million grasps. Beyond benchmarking, we also propose a novel two-stage grasping method that learns efficiently from data by using a diffusion model that conditions on local geometry. Our proposed generative method outperforms all baselines in simulation experiments. Furthermore, with the aid of test-time-depth restoration, our method demonstrates zero-shot sim-to-real transfer, attaining 90.7% real-world dexterous grasping success rate in cluttered scenes.

==> sections/supp99_Video.tex <==
\section{[describe our supp video]}

==> tables/grippers_old.tex <==

\begin{table}[t]\tiny
    \centering
    \begin{tabular}{p{13mm}|>{\centering}m{8mm}>{\centering}m{8mm}>{\centering}m{11mm}|>{\centering}m{8mm}>{\centering}m{8mm}>{\centering}m{11mm}|>{\centering}m{8mm}>{\centering}m{8mm}c}
    \toprule
    
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Seen} & \multicolumn{3}{c|}{Similar} & \multicolumn{3}{c}{Novel} \\
    
    \cline{2-10}
    & \textbf{AP} & AP$_{0.8}$ & AP$_{0.4}$ & \textbf{AP} & AP$_{0.8}$ & AP$_{0.4}$ & \textbf{AP} & AP$_{0.8}$ & AP$_{0.4}$ \\

    \hline
    GG-CNN~\cite{morrison2018closing} & 15.48/16.89 & 21.84/22.47 & 10.25/11.23 & 13.26/15.05 & 18.37/19.76 & 4.62/6.19 & 5.52/7.38 & 5.93/8.78 & 1.86/1.32 \\

    Chu \textit{et al.}~\cite{chu2018real} & 15.97/17.59 & 23.66/24.67 & 10.80/12.74 & 15.41/17.36 & 20.21/21.64 & 7.06/8.86 & 7.64/8.04 & 8.69/9.34 & 2.52/1.76 \\

    GPD~\cite{ten2017grasp} & 22.87/24.38 & 28.53/30.16 & 12.84/13.46 & 21.33/23.18 & 27.83/28.64 & 9.64/11.32 & 8.24/9.58 & 8.89/10.14 & 2.67/3.16 \\

    PointGPD~\cite{liang2019pointnetgpd} & 25.96/27.59 & 33.01/34.21 & 15.37/17.83 & 22.68/24.38 & 29.15/30.84 & 10.76/12.83 & 9.23/10.66 & 9.89/11.24 & 2.74/3.21 \\

    GraspNet1B~\cite{fang2020graspnet} & 27.56/29.88 & 33.43/36.19 & 16.95/19.31 & 26.11/27.84 & 34.18/33.19 & 14.23/16.62 & 10.55/11.51 & 11.25/12.92 & 3.98/3.56 \\

    GSNet~\cite{wang2021graspness} & 67.12/63.50 & 78.46/74.54 & 60.90/58.11 & 54.81/49.18 & 66.72/59.27 & 46.17/41.89 & 24.31/19.78 & 30.52/24.60 & 14.23/11.17 \\

    \hline
    Ours &  &  &  &  &  &  &  &  &  \\
    
    \hline
    Ours (refine) &  &  &  &  &  &  &  &  &  \\
    
    Ours (render) & 84.5 &  &  & 78.4 &  &  & 44.6 &  &  \\
    
    Ours (1/10) & 82.1 &  &  & 76.4 &  &  & 42.2 &  &  \\
    
    \bottomrule
    \end{tabular}


    \caption{GraspNet-1Billion evaluation results on RealSense/Kinect. \textit{\textbf{Refine}} uses 4.2M refined grasp labels. \textit{\textbf{Render}} uses 4.2M refined grasp labels and rendered depth images. \textit{\textbf{1/10}} uses 420K randomly subsampled refined grasp labels and rendered depth images. \liuhaoran{fill table}\liuhaoran{train gs net on friction 0.2, compared with flow on friction 0.2}}

    \label{tab:gripper}
\end{table}
